The algorithmic nature of song-sequencing: statistical regularities in music albums

Based on a review of anecdotal beliefs, we explored patterns of track-sequencing within professional music albums. We found that songs with high levels of valence, energy and loudness are more likely to be positioned at the beginning of each album. We also found that transitions between consecutive tracks tend to alternate between increases and decreases of valence and energy. These findings were used to build a system which automates the process of album-sequencing. Our results and hypothesis have both practical and theoretical applications. Practically, sequencing regularities can be used to inform playlist generation systems. Theoretically, we show weak to moderate support for the idea that music is perceived in both global and local contexts.

==> notes.tex <==

% (https://www.bbc.co.uk/sounds/play/b01q95y6)
%     - In an interview to the Rolling Stone magazine, Barry Hefner \footnote{co-founder of the record label \textit{SinceThe80s}}, suggests that positioning the most impactfull tracks in the beginning of the albums is especially relevant for "new and younger artists that are trying to capture the attention of an audience".

% Finally, global perspectives do not need to reside within the barriers of a single composition. Essentially  From that perspective, it would be possible to test both global and concatenationist hypothesis in the context of any musical sequence (e.g. playlists, albums, DJ sets and concerts). 

% In our investigation of PMAs, we explore sequential patterns that may reflect global or local biases on track sequencing. It might be the case, for instance, that the album presents a clear global structure between its first and its last track (e.g. tracks present a linear trend of increasing loudness). Conversely, we might find that there are transitional patterns only between consecutive tracks, (e.g., a loud track follows a soft one). Before we consider this in more detail, we review yet another set of studies that can also offer some insight into the questions that we ask here.


%  Still, in order to challenge the concatenationist view of music perception, one would not have to demonstrate that listeners apprehend the tonal hierarchies of a \textit{sonata-allegro}, for instance. Rather, if we find that tracks are differently perceived depending on the order in which they appear in an album, this could also be indicative of  global account of music perception. From this perspective, it is possible to extend the global/local discussion to the context of albums and playlists.

% anecdotal beliefs

% \cite{ruoff2018how}
% try to ensure that you don't play more than 2 similar songs in a row to keep your playlist exciting.

% Structure the playlist like a flight
% Generally speaking, a plane takes off, stays in the air for a bit, and then gently comes down. That's the arc you want to build your playlist around.

% https://www.wikihow.com/Make-an-Awesome-Music-Playlist#Organizing-Songs
% Start with a hook. Whatever your theme, genre, or taste, one thing about playlists is universal: it's got to start with a great song. Lead off with a song that'll hook everyone who'll listen.

% https://community.spotify.com/t5/Archived-Chat/How-To-Make-A-Good-Playlist/m-p/4580494
% Although the order of songs doesn’t always matter, try to grab passers-by attention straight the way by making sure the first 10 songs are straight bangers

% \cite{ruth2019how}
% When you have a group of songs that are of a similar style, get to know how upbeat or slow each song is. You could try and alternate quicker and slower tempo songs or vary the mood.

% \cite{sawyer2021how}
% The trick is to make sure each song is there for a reason. A good playlist should flow from start to finish in the same way a full album or individual song is meant to. 


% https://www.youtube.com/watch?v=en3HYS7R9DQ (beginning is important)
% https://www.youtube.com/watch?v=Z6zGMIZgP24 (contrast is important; beginning is important; spread out tempo and key)

% \cite{friedman2021how}
% on average, albums start off with a slightly faster-than-average song, and end with slightly slower-than-average songs. There’s a small tempo dip at the third decile, and upticks in tempo at the 4th and 6th deciles. 

